Detecting Manipulated Contents Using Knowledge-Grounded Inference

The detection of manipulated content, a prevalent form of fake news, has been widely studied in recent years. While existing solutions have been proven effective in fact-checking and analyzing fake news based on historical events, the reliance on either intrinsic knowledge obtained during training or manually curated context hinders them from tackling zero-day manipulated content, which can only be recognized with real-time contextual information. In this work, we propose Manicod, a tool designed for detecting zero-day manipulated content. Manicod first sources contextual information about the input claim from mainstream search engines, and subsequently vectorizes the context for the large language model (LLM) through retrieval-augmented generation (RAG). The LLM-based inference can produce a "truthful" or "manipulated" decision and offer a textual explanation for the decision. To validate the effectiveness of Manicod, we also propose a dataset comprising 4270 pieces of manipulated fake news derived from 2500 recent real-world news headlines. Manicod achieves an overall F1 score of 0.856 on this dataset and outperforms existing methods by up to 1.9x in F1 score on their benchmarks on fact-checking and claim verification.

==> sections/abstract.tex <==
% !TeX root = ../main.tex

The detection of fake news, a type of misinformation that could significantly impact society, has been widely studied in recent years.\RW{remove texts between , and ,?} Nonetheless, most existing approaches to recognizing fake news from the facts are based on machine learning classifiers that usually request a large amount of high-quality labeled training data and are, therefore, incapable of tackling first-hand recent fake news.
\MX{I didn't get the connection:
why the requirement on labeled data make these models
incapable of tracking first-hand manipulated content?}

In this work, we are inspired by the most recent progress of large language models (LLMs), which have demonstrated excellent natural language comprehension and generation capabilities, to design a fake news detection solution by leveraging the state-of-the-art LLMs.\RW{In this work, we leverage large language models (LLMs) to design a fake news detection solution.}
\MX{I am in favor of Ruizhe's version}.
%
Our method consists of three steps, namely online knowledge retrieval, context construction, and knowledge-grounded inference by LLMs. 
Specifically, it first searches the input statement on mainstream search engines on the Internet to source relevant information. 
The search results about the user's input are treated as knowledge and are vectorized as the context for LLM inference through the lens of retrieval-augmented generation (RAG). 
Our LLM-based inference can produce a truth or fake news decision and offer a justification to explain it. Through a real-world news headline dataset, we demonstrate that the outstanding performance of our approach in detecting fake news about recently happened events around the world.

\MX{Rewriting work-in-progress}
The detection of manipulated content,
a type of mis- and disinformation,
has been widely studied in recent years.
%
\MX{I need to examine the related works
for any new propositions, candidate include: \\
\\
- these models focus on all types of mis/dis info (including "fabricated" content)
  while we only focus on "manipulated".
  This has an advantage, as by definition, "manipulated" content
  has a base which can serve as extra input. \\
  \\
- these models suffer from the aging problem, i.e.,
  they perform well on manipulated content based on historical information,
  but not on manipulated content on new information
  that is not index in their training data. \\
}

\MX{@Mark, can you help validate the above propositions?}



==> sections/abstract_1.tex <==
% !TeX root = ../main.tex

The detection of manipulated content---a type of fake news---has
been widely studied in recent years. 
%
While existing solutions have been proven effective
in fact-checking and analyzing fake news based on historical events,
the reliance on
either intrinsic knowledge obtained during training
or manually curated context
hinders them from tackling zero-day manipulated content
which can only be recognized with real-time contextual information.

In this work,
we propose a tool, \toolname, that focuses on
(zero-day) manipulated content detection.
%
\toolname first source contextual information
about the input claim from mainstream search engines,
and subsequently vectorize the context for the LLM through RAG.
%
The LLM-based inference can produce a
``integral'' or ``manipulated'' decision and
offer a textual explanation for the decision.
%
To validate the effectiveness of \toolname,
we also propose a dataset consisting of over 4270 pieces of fake news
that are manipulated based on \allnewscollected recent real-world news headlines.
%
\toolname achieves an overall F1 score of \ourfone
on the new dataset and
outperforms existing works by up to 1.9x in F1 score
on their benchmarks on fact-checking and claim verification.


==> sections/intro.tex <==
% !TeX root = ../main.tex

\section{Introduction}
\label{sec:intro}

The widespread of fake news on the Internet has become a major concern in recent years.
Fake news \MX{Let's use \emph{manipulated content},
as defined in~\autoref{sec:terms}
instead of fake news throughout the paper},
as a type of misinformation, is usually produced by making minor but misleading modifications to the truth. Fake news generated with malicious intentions could bring tremendous harm to the unity and harmony of society and often requires a large amount of manpower and resources to be clarified. For those reasons, how to precisely and effectively detect fake news from mass information has become a widely studied problem in the research community. 

Although there are many prior works on fake news detection, most existing approaches are implemented based on a machine learning classifier~\cite{nie2019combining,ma2019sentence,popat2018declare,wu2021evidence}, and therefore, heavily rely on the training process. They only work well with high-quality labeled data and through a well-trained classifier model \RW{work well with that has been classifier model that has been trained with high-quality labeled data?}.
Unfortunately, most fake news drastically threading to our society are about zero-day or most recently happening events,
\MX{I don't know how to interpret the text.
%
Here is the ML model I can naively imagine
for the "manipulated content" detection problem: \\
%
- Input 1: news to be questioned \\
- Input 2: context gathered about the news to be questioned \\
- Output: label (and potentially a reasoning) \\
%
The questions I have is: \\
1) Is there related work following this line of model? \\
2) Is there any intuition on why they would perform bad on zero-day manipulated content?
}
on which existing approaches are commonly incapable to well handle. How to effectively detect fake news about most recent contexts, remains an open question.

In this work, we are inspired by the most recent progress of large language models (LLMs), which have demonstrated excellent capabilities in natural language comprehension and generation and, therefore, have been substantially applied in fact-checking tasks~\cite{lee2021towards,wang2023explainable}.
\MX{This is probably the LAST reason a reviewer want to see.
%
You should NEVER say that you adopt a new thing
because it is cool or
because everyone else is doing it, instead,
you SHOULD argue from the perspective that
LLMs, with their capabilities in natural language comprehension and generation, either
solves a core problem or
addresses a fundamental weakness / missing piece in prior approaches.
%
Now, question for @Mark, what is this
problem / weakness / missing piece LLMs fit in?}
%
We design a fake news detection solution by leveraging the state-of-the-art LLMs.
%
Our method consists of two steps,
\MX{this is not consistent with what is mentioned in abstract.
In abstract, our method consists of **three** steps:
online knowledge retrieval,
context construction, and
knowledge-grounded inference by LLMs}
namely online searching and LLM inference. It first searches an input on mainstream search engines on the Internet to source relevant information, followed by the LLMs’ inference based on the relevant information. To address the limitation of token numbers in a conversational session with LLMs, we adopt the retrieval-augmented generation (RAG) technique to encode the relevant information into a vector database. Moreover, in addition to a truth or fake decision, our approach takes advantage of the powerful natural language understanding capabilities of LLMs to offer a justification.

Our approach is evaluated with a real-world news headline dataset, and the experimental outcomes demonstrate outstanding performance in detecting fake news about recently happened events around the world, with an overall precision of 90.9\% and a recall rate of 84.6\%.

\MX{In security conferences,
it is usually a customary to have a summary (list) of contributions,
do we need this for WWW?}\\
\menghs{Yes, let me add them later}

\begin{figure}[t]
	\centering
	\includegraphics[width=1\linewidth]{figures/running-example.pdf}
	\caption{A running example of our proposed fake news detection to detect and analyze simulated first-hand fake news as of 2024 Jul 29, with factual mistakes in the user queries underlined in red, and key explanations offered by our system underlined in black.}
	\label{fig:running-example}
\end{figure}

==> sections/literature_review.tex <==
% !TeX root = ../main.tex

\section{Background}

\subsection{Disinformation and Misinformation}
\label{sec:terms}

Disinformation describes content that is intentionally false and designed to cause harm.
It distinct from \emph{misinformation} or \emph{false information} in a broader sense, that disinformation is falsified based on truth and involves malicious intent to mislead people and induce audience to believe, while misinformation and false information do not have to do so~\cite{zurko2022disinformation}. 

Combating disinformation has been a widely recognized challenge in nowadays society. 
Agents of disinformation have learned that using genuine content and reframing it in misleading but indistinguishable ways is less likely to be detected by existing AI systems~\cite{wardle2020understanding}.
The harm of disinformation is often amplified during the dissemination where people may sharing it their social networks without realizing it is false and even believing that it is helpful.

The study on disinformation involves not only computer science community but also political, journalism, and socio-psychology researchers. 
Zurko~\cite{zurko2022disinformation} reviews the evolution of disinformation and misinformation since 1970s and outlook the technological development for combatting disinformation from the usable security perspective.
Mazurczyk et al.~\cite{mazurczyk2024disinformation} share their opinions on leveraging AI techniques in building a holistic solution to counter disinformation.
Wardle~\cite{wardle2020understanding} in his book established a set of taxonomy to reveal the spectrum of disinformation. 
Seven categories of disinformation have been proposed based on the different intentions and the extent of fabrication over the ground truth. According to that spectrum, the scope of disinformation ranges from intelligent satire and parody, to information with misleading or manipulated content, and eventually to completely fabricated contents.
In this paper, we do target the motivation behind the production and dissemination of disinformation, such as being it for fun or for profit, propaganda, sponsorship, or just an honest mistake. We also assume the disinformation circulating on the Internet is unlikely completely fabricated without being partially backed with the ground truth because it would be easy for AI system to detect.
Instead, we focus on disinformation in form of a text that contains minor or indistinguishable perturbations, with all remaining parts being truth to circumvent the mainstream AI fact-checking or relevant mechanism.

\subsection{Disinformation Detection}
\label{sec:literature_review}

\MX{Following~\autoref{sec:terms}, as well as is mentioned in Introduction,
it might be a good idea to discuss the problem setup before discussing any
concrete solutions. \\
%
Now, you can choose to abstract either \\
- manipulated content detection or \\
- mis- and disinformation detection \\
as a blackbox and present how each related work in the literature fill in this black box.}

\MX{Regardless of which level of abstraction you choose from,
as a blackbox, please just focus on
1) what is the input, and 2) what is the output.}

\MX{After presenting the problem statement (as a blackbox),
we can start to talk about how this blackbox is implemented in the literature.
And this can be effectively done by **categorizing existing works**
based on their techniques,
for example
(of course I haven't read much of related works, this is just to show the organization): \\
- classification based on unique features in manipulated content or mis- and disinformation \\
- <I have no idea what sentence-level embedding for claim verification~\cite{ma2019sentence} is> \\
- <what is unique about Lu et al.~\cite{lu2020gcan}?> \\
- <what is unique about Nie et al.\cite{nie2019combining}?> \\
- <what is fundamentally operated on by Lee et al.~\cite{lee2021towards}?,
   in other words, why BERT and LLM can even help in the Lee et al.~\cite{lee2021towards} case?> \\
- <what is this chain-of-thought mechanism of LLM~\cite{wang2023explainable} doing?
  And why this is in the picture?>
- <what is this competing wisdom~\cite{wang2024explainable} doing?>
}

\paragraph{Fake News Detection by Conventional Machine Learning Models}
Fake news detection has been studied in the research community for decades. Early approaches mostly leverage conventional machine learning classification to predict if a statement is true or fake. Considering the lack of powerful natural language comprehension solutions in the early years, the prior study mainly distinguished fake news from truth through the lens of feature engineering. For example, fake news is widely regarded have obvious differences with truth in terms of salient phrases~\cite{popat2018declare,wu2021evidence} or news attributes~\cite{yang2019xfake}. In addition to merely making predictions, the research community has also put persistent effort into producing explanations, therefore achieving explainable fake news detection~\cite{shu2019defend}. Ma et al.~\cite{ma2019sentence} leverage hierarchical attention networks to propose sentence-level embedding for claim verification. Lu et al.~\cite{lu2020gcan} adopt a graph neural network to construct a justification for detecting fake news circulating in social networks. Nie et al.~\cite{nie2019combining} investigate the usage of neural semantic matching networks in providing justification along with fake news prediction. 

\paragraph{Fake News Detection in LLM-era}
After the debut of the BERT model family, the research community started exploring the adoption of LLMs in solving the fact-checking problem. Lee et al.~\cite{lee2021towards} train a few BERT-based LLMs for fact-checking, and propose two COVID-related datasets for benchmarking purposes, demonstrating the powerful capabilities of LLMs in claim reasoning for the first time. Wang et al.~\cite{wang2023explainable} explore leveraging the chain-of-thought mechanism of LLM in fact verification reasoning. Wang et al.~\cite{wang2024explainable} propose explainable fake news detection with LLMs via defense among competing wisdom. Although it still resorts to conventional machine learning models to classify the input claim, their approach innovatively leverages LLMs to reason competing evidence to construct a control group, i.e., competing wisdom, and therefore to facilitate final predictions. Their method has achieved state-of-the-art performance; however, its wisdom can only be built based on a pre-defined knowledge base, making it incapable of handling fake news that has recently happened. Our work leverages online search engines to proactively search supportive documents, and therefore, can effectively detect zero-day or recently happened fake news.

==> tables/benchmarking_baseline_binary_transpose.tex <==
% !TeX root = ../main.tex

\begin{table}[t]
\centering
% Config the row spacing
\def\arraystretch{1.01}
% Config the column spacing
\setlength{\tabcolsep}{3pt}
\caption{Benchmarking outcomes (comparison with binary label automatic fact checking~\cite{lee2021towards}) \label{tab:benchmarking_binary_sota}}
\vspace{0cm}
\footnotesize
\begin{tabular}{lrcccc}
\hline  
  &  & XLNet\textsubscript{\textit{ft}} & BERT\textsubscript{\textit{PPL}} & GPT2\textsubscript{\textit{PPL} (15b)}  & Ours  \\ \hline
COVID~\cite{google2024bigbench} & Accuracy & 0.632  & 0.625  & 0.783  & 0.873 \\ \cline{2-6}
  & F1 score  & 0.520  & 0.611  & 0.776  & 0.911 \\ \hline
FEVER~\cite{thorne2018fever} & Accuracy & 0.492  & 0.574  & 0.736  & 0.807 \\ \cline{2-6}
  & F1 score  & 0.484  & 0.569  & 0.717  & 0.788 \\ \hline  
\end{tabular}
\end{table}

==> tables/benchmarking_baseline_multilabel_transpose.tex <==
% !TeX root = ../main.tex

\begin{table*}[t]
\centering
% Config the row spacing
\def\arraystretch{1.01}
% Config the column spacing
\setlength{\tabcolsep}{3pt}
\caption{Benchmarking outcomes (comparison with multi-label fact checking) \label{tab:benchmarking_multilabel_sota}}
\vspace{0cm}
\footnotesize
\begin{tabular}{lrccccHcccHccHc}
	\hline  
&  &  \multicolumn{4}{c}{Traditional Approaches} & & \multicolumn{3}{c}{LLM-based Approaches} & & \multicolumn{2}{c}{Defense-based w. LLM} & & \\ 
\cline{3-6}\cline{8-10}\cline{12-13}
%\cmidrule(r){3-6}\cmidrule(r){7-9}\cmidrule(r){10-11}
&  & dEFEND~\cite{shu2019defend} & SBERT-FC~\cite{kotonya2020explainable} & GenFE-MT~\cite{atanasova2020generating} & CofCED~\cite{yang2022coarse} & &
  LLaMA2~\textsubscript{claim}~\cite{ouyang2022training} & 
  ChatGPT\textsubscript{claim}~\cite{ouyang2022training} & FactLLaMA\textsubscript{know}~\cite{cheung2023factllama}  & & L-Defense\textsubscript{LLaMA2}~\cite{wang2023explainable}  & L-Defense\textsubscript{ChatGPT}~\cite{wang2023explainable} & & Ours \\ \hline
& Precision & 0.231  & 0.241  & 0.186  & 0.295  & & 0.171  & 0.254  & 0.325  & & 0.316  & 0.306  & & 0.920  \\ \cline{2-15}
LIAR-RAW  & Recall  & 0.186  & 0.221  & 0.199  & 0.296  & & 0.174  & 0.273  & 0.321  & & 0.317  & 0.322  & & 0.910  \\ \cline{2-15}
  & F1 Score  & 0.175  & 0.222  & 0.152  & 0.289  & & 0.151  & 0.251  & 0.304  & & 0.314  & 0.305  & & 0.915  \\
\hline  
& Precision & 0.449  & 0.511  & 0.456  & 0.530  & & 0.373  & 0.477  & 0.561  & & 0.610  & 0.617  & & 0.821  \\  \cline{2-15}
RAWFC & Recall  & 0.433  & 0.459  & 0.453  & 9.510  & & 0.380  & 0.486  & 0.555  & & 0.600  & 0.610  & & 0.932  \\  \cline{2-15}
& F1 Score  & 0.441  & 0.455  & 0.451  & 0.511  & & 0.368  & 0.444  & 0.557  & & 0.601  & 0.612  & & 0.873 \\ \hline  
\end{tabular}
\end{table*}

==> tables/news_dist_dbl_col.tex <==
% !TeX root = ../main.tex

\begin{table}[t]
\caption{Distribution of the news in our dataset \label{tab:news_dist}}
\begin{tabular}{ll}
\hline
\multicolumn{2}{l}{Distribution by Regions} \\\hline
Singapore                         & 42      \\
Canada                            & 19      \\
Oceania \& South Africa           & 43      \\
UK                                & 135     \\
US \& Worldwide                   & 67      \\\hline
                                  &         \\\hline
\multicolumn{2}{l}{Distribution by News Providers}  \\\hline
BBC                               & 115     \\
New York Times                    & 10      \\
FOX News                          & 13      \\
Google News                       & 168     \\\hline
                                  &         \\\hline
Total                             & 306     \\\hline
     
\end{tabular}
\end{table}

==> tables/news_dist_single_col.tex <==
% !TeX root = ../main.tex

\begin{table}[t]
\centering
% Config the row spacing
\def\arraystretch{1.03}
% Config the column spacing
\setlength{\tabcolsep}{1pt}
\caption{Distribution of the news collected \label{tab:news_dist}}
\vspace{-0.3em}
\footnotesize

\resizebox{\linewidth}{!}{%
\begin{tabular}{lrllrllr}
\cline{1-5}\cline{7-8}
\multicolumn{5}{c}{\textbf{Distribution by Regions}} &  & \multicolumn{2}{c}{\textbf{Distribution by News Providers \quad}} \\
\cline{1-5}\cline{7-8}
US \& Worldwide & 995 && Australia & 205 & 
& Google News & 1444 \\
UK & 533 && South Africa & 176 &
& BBC & 443 \\
Canada & 230 && New Zealand & 147 & 
& New York Times & 328 \\
Singapore & 214 & & & &
& Fox News & 285\\ \cline{1-5}\cline{7-8}
\textit{Total} & & & & \allnewscollected &
& \textit{Total} & \allnewscollected \\\cline{1-5}\cline{7-8}
\end{tabular}
}
\end{table}

==> tables/true_and_fake_news_dict.tex <==
% !TeX root = ../main.tex

\begin{table}[t]
\centering
\caption{Distribution of the news collected \label{tab:dataset_dist}}
\begin{tabular}{lr}
\hline
\textbf{Type} & \textbf{Quantity} \\\hline
True News ($X$) & \alltruenews \\ 
Fake News (Negative Sentiment, $X_n$) & \allfakeneg \\ 
Fake News (Altered Context, $X_c$) & \allfakectx \\\hline 
\textit{Total} & 567 \\ \hline
\end{tabular}
\end{table}

==> tables/veracities_prediction_performance.tex <==
% !TeX root = ../main.tex
% \usepackage{multirow}

\begin{table}[t]
\centering
\caption{The confusion matrix of our veracity performance evaluation \label{tab:confusion_matrix}}
\small
\begin{tabular}{llrr}
\hline
 & & \multicolumn{2}{c}{Predictions} \\\cline{3-4}
 & & \multicolumn{1}{c}{Positive (Disinfo.)} & \multicolumn{1}{c}{Negative (Truth)} \\\hline
\multicolumn{1}{c}{\multirow{2}{*}{Fact}} & \multicolumn{1}{c}{Fake}  & \tpcases & \tncases \\\cline{2-4}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{True} & \fpcases & \fncases \\\hline
\end{tabular}
\end{table}
